Reconstructing Embedded Graphs from Persistence Diagrams

The persistence diagram (PD) is an increasingly popular topological descriptor. By encoding the size and prominence of topological features at varying scales, the PD provides important geometric and topological information about a space. Recent work has shown that well-chosen (finite) sets of PDs can differentiate between geometric simplicial complexes, providing a method for representing complex shapes using a finite set of descriptors. A related inverse problem is the following: given a set of PDs (or an oracle we can query for persistence diagrams), what is underlying geometric simplicial complex? In this paper, we present an algorithm for reconstructing embedded graphs in $\mathbb{R}^d$ (plane graphs in $\mathbb{R}^2$) with $n$ vertices from $n^2 - n + d + 1$ directional (augmented) PDs. Additionally, we empirically validate the correctness and time-complexity of our algorithm in $\mathbb{R}^2$ on randomly generated plane graphs using our implementation, and explain the numerical limitations of implementing our algorithm.

==> body/append-transcription.tex <==
\section{Transcription of PHT Paper}
\todo{describe the edge reconstruction in terms of reconstructing a 1-complex in
$\R^2$, as a direct transcription of the Turner paper.}

\brittany{ah, ... I remember this one!  Turner et al. do present a
`reconstruction' but we never figured out what it was. If possible, we should
figure it out and include that in this paper.  Please remind me to email her
early this week.  Also, who would like to be charged with this task?}
\anna{Why is it necessary to transcribe a paper to which we have already
included a reference?}


==> body/onepoint.tex <==
%%%%% Technical details %%%%%%]
\begin{lemma}[Location of a Point]
	Let $\simComp$ be a simplicial complex composed of a single vertex
    $p\in \R^2$.
    Let $\dir_1, \dir_2 \in \sph^1$ be pairwise linearly independent.
    Let $\hFilt{\dir_1}$ and $\hFilt{\dir_2}$ be height filtrations
    from directions $\dir_1$ and $\dir_2$ respectively.
    The $(x,y)$ coordinates of $p$ can be computed using the zero-dimensional
    persistence diagrams $\dgm{0}{\dir_1}$ and $\dgm{0}{\dir_2}$ resulting from $\hFilt{\dir_1}$ and
    $\hFilt{\dir_2}$ on $\simComp$.
    \label{lem:pointLoc}
\end{lemma}
\begin{proof}
The height filtrations $\hFilt{\dir_1}$ and $\hFilt{\dir_2}$ will
encounter $p$ at a unique height.
Since $p$ is the only point in $\simComp$, $D_1$ and $D_2$ will
be composed of exactly one feature each corresponding to
the point $p$.
Then, $\pLines{\dir_1}{p}$ and $\pLines{\dir_2}{p}$ are each composed
of a single line representing the birth event of $p$ in $\dgm{0}{\dir_1}$ and
$\dgm{0}{\dir_2}$ respectively.
Since, $\dir_1$ and $\dir_2$ are linearly independent,
these lines are not parallel.
Therefore, they intersect at exactly one point.
Assume that $p$ does not lie at the point where the lines intersect.
Then, one of the
height filtrations must not have encountered $p$ at the
the height where the line corresponding to the birth lies because this line
does not intersect with $p$, a contradiction.
Therefore, the $(x,y)$ coordinates for the intersection of the two lines from
$\pLines{\dir_1}{p}$ and $\pLines{\dir_2}{p}$ are the $(x,y)$ coordinates for $p$.
\end{proof}



